Uncertainty-Aware Acoustic Localization and Mapping for Underwater Robots

For underwater vehicles, robotic applications have the added difficulty of operating in highly unstructured and dynamic environments. Environmental effects impact not only the dynamics and controls of the robot but also the perception and sensing modalities. Acoustic sensors, which inherently use mechanically vibrated signals for measuring range or velocity, are particularly prone to the effects that such dynamic environments induce. This paper presents an uncertainty-aware localization and mapping framework that accounts for induced disturbances in acoustic sensing modalities for underwater robots operating near the surface in dynamic wave conditions. For the state estimation task, the uncertainty is accounted for as the added noise caused by the environmental disturbance. The mapping method uses an adaptive kernel-based method to propagate measurement and pose uncertainty into an occupancy map. Experiments are carried out in a wave tank environment to perform qualitative and quantitative evaluations of the proposed method. More details about this project can be found at https://umfieldrobotics.github.io/PUMA.github.io.

==> sections/Discussion.tex <==
% \subsection{Disturbance Characterization on Acoustic Sensors}
%     We propose an experiment for characterizing the induced noise on acoustic sensors due to dynamic pressure from wave conditions, as it is common in many environments of AUVs.
%     We hypothesize that acoustic-based sensors will be prone to inaccurate readings when operating near the surface in environments with wave conditions.
%     We utilize prior knowledge obtained from coastal and wave dynamics literature regarding the dynamic pressure profile under wavy conditions \cite{bosboom_coastal_2021} .
%     As the wave oscillates and wave height $z$ changes, the added dynamic pressure on the hydrostatic pressure experienced by the sensor also oscillates.
%     The dynamic pressure generated can then be characterized as shown in $\hat{p}$ in Eqn. \eqref{eq:dynamic_pressure}, where $h$ represents the depth underwater, $k$ the wave number, and $\rho_W$ the density of water.
%     \begin{gather}
%         p_{\text{total}} = p_H + \hat{p} \\
%         p_H = \rho_W gh \label{eq:hydrostatic_pressure}\\
%         \hat{p} = \frac{\rho_W gh}{2}\frac{\cosh k\left(h+z\right)}{\cosh kh}
%         \label{eq:dynamic_pressure}
%     \end{gather}
%     As the pressure of the medium in which the acoustic signals vary, the density of the medium similarly changes, impacting the speed at which acoustic signals are transmitted.
%     For the DVL, this relates to a shift in the Doppler shift, which is used for measuring the speed of the body frame, while for sonars, this translates to a change in the time of flight of the signal, impacting the distance measurement made.
%     \newline
%     \indent The results obtained from our tests are used to validate these assumptions.
%     Table \ref{tab:wave_table} provides quantitative results on the standard deviation of the measurements at the times when waves were operating.
%     We claim that the origin of these deviations is the oscillatory dynamic pressure induced by the waves; hence, it is considered the measurement noise of the sensors at the time of induced waves.
%     \newline
%     \indent We highlight that there are observed differences in the measurement noise of the velocity and altitude measurements from the DVL, justifying the inclusion of the additive noise in the state estimation formulation.
% \subsection{State Estimation Performance}
%     We present a state estimation method with two key contributions to reducing drift and accounting for disturbance induced by environmental factors. The bias estimation is formulated as a random walk \cite{haessig_separate-bias_1998}, and the predicted bias term at each time step is accounted for in the measurement model of the filtering step. \newline
%     \indent The disturbances induced by the waves are empirically evaluated using an experiment set up in a wave pool. The deviation on the sensor readings is used as added noise in the measurement model in the filtering formulation. It is added to reduce trust in the sensor measurements when waves are induced.
%     \newline
%     \indent We observe two distinct effects of each factor on the state estimation and use this section to analyze their impact.
%     \subsubsection{Impact of Bias Estimation on the State Estimation}
%         The bias estimation and correction in the filtering output directly estimate the robot's heading correction during its operation. We see from the results obtained from the ablation study in Table \ref{tab:ablation} that this bias correction accounts for a significant correction for the drift of up to 25 cm over 36.6 m of travel. In addition, we show that the heading correction is improved, a critical factor in reducing the drift over extended operations of the robot. 
%     \subsubsection{Impact of Added Noise on the State Estimation}
%         The most significant contribution of the added noise is to the velocity estimates of the AUV, which is the observable state variable that is impacted by the additive noise. 
%         This is most apparent in the scaled additive noise, where there is a lower root mean squared error on the velocity estimates.
%         Despite the increased accuracy in the velocity over the robot's operation, we observe that the pose estimate degrades when compared to the baseline. 
%         We hypothesize that this occurring on the pose estimation error is related to a bias on the velocity measurements when the waves are induced to the system.
%         \newline 
%         \indent From observations of the measurements taken during the wave tests, we observed a persistent bias in the sensor measurements that the DVL was making.
%         This observed bias is shown in Fig. \ref{fig:velocity_bias}, where the ground truth, measured, and estimated velocity are in the $x$-direction in the robot frame.
%         We hypothesize that this incorrect velocity measurement in the $x$-direction is a key factor in the large RMSE on the $x$-position.

% \subsection{Mapping Performance}
%     We propose an adaptive BKI mapping solution. 
%     We decompose the original kernel in ~\cite{doherty2019learning} that conducts radius ball search into $3$ separate kernels. In addition, we make the length scales adaptive to the state uncertainty.
%     As we propagate the filter for the state estimation, the uncertainties of the robot state at the $x-y$ plane gradually increase as there is no direct measurement for the robot's $x-y$ positions. 
%     In contrast, the uncertainty of the depth of the robot is maintained constantly low due to the pressure sensor. 
%     This results in different orders of magnitude for uncertainties in the $x-y$ plane and the $z$-axis. 
%     \newline
%     \indent After decomposing the kernels, we can properly propagate the relatively larger state uncertainty in the $x-y$ plane while maintaining a more strict threshold in the $z$-axis. 
%     Theoretically, when the lengthscale in an axis increases, for a single range measurement, it informs that more neighboring map points in that axis might be occupied with a less centralized kernel value map, according to Eqn. \eqref{eq:kernel}, which shows reduced confidence in the occupancy of the surrounding map points.
%     \newline
    % \begin{figure}
    %     \centering
    %     \captionsetup{justification=centering}
    %     \includegraphics[width=0.95 \linewidth]{figures/rviz_robot.pdf}
    %     \caption{Visualization using RViz of the robots projected range measurements made from the DVL (red rays) and Ping Sonar (gray ray). Additionally, the green points represent map points captured by a dense LiDAR when the tank is drained. The constructed map is used as the ground truth map for evaluating methods.}
    %     \label{fig:rviz_robot}
    % \end{figure}
    % \begin{figure}
    %     \centering
    %     \captionsetup{justification=centering}
    %     \includegraphics[width=0.9 \linewidth]{figures/3d map.pdf}
    %     \caption{A visualization of the map constructed from the presented method. The black point cloud represents the dense LiDAR scan obtained in the emptied tank for ground truth, and the red-to-blue colored points represent the constructed occupancy map using our method. The color map of the occupancy map represents the distance error, low being blue and high being red.}
    %     \label{fig:map_qualitative}
    % \end{figure}
    % \indent In Table \ref{tab:mapping_results}, we can see that with the proposed state estimation method, the mapping accuracy is significantly improved. It is also demonstrated that the BKI mapping algorithm is capable of generating denser mapping algorithms than the CSM method. It is noted that with our proposed adaptive kernel method for state uncertainty propagation, the number of occupied cells is reduced. We argue that larger number of occupied cells does not necessarily improve the map quality. For fair comparison, we set the lengthscale of the BKI method to be $0.15$m so the radius ball search covers similar volume as our proposed mapping method with the largest lengthscales along the three axes. Therefore, the baseline BKI method marks more cells to be incorrectly occupied when the state uncertainty is small. Besides, as our state estimation algorithm maintains direct measurement over $z$ with the pressure sensor, the mapping algorithm should be more strict on the $z$ axis due to smaller uncertainty in that direction. As shown in Fig. \ref{fig:map_comparison}, our method effectively takes this benefit from the pressure sensor into account, while the baseline BKI method lacks adaptivity handling the imbalanced uncertainties along different axes, which results larger error in its mapping accuracy.

    

==> sections/drafts.tex <==
% \subsubsection{Unscented  Kalman Filter}
% The Unscented Kalman Filter (UKF) is a Gaussian filtering method that utilizes quadrature integration in order to approximate the integrals of the Bayes filtering steps \cite{zheng_unscented_2019} by defining sigma points $\mathcal{X}$ and weights $w$ to use in a weighted sum, as shown in \eqref{eq:quadrature}.
% \begin{gather}
%     \int h(x)dx \approx \sum_i h(\mathcal{X}^{(i)})w^{(i)} \label{eq:quadrature}
% \end{gather}
% For the state vector $\mathbf{x} \in \mathbb{R}^d$, the sigma points are defined as $2d+1$ basis vectors, as shown in eq. \eqref{eq:sigma_points}, with weights defined according to the rule in eqs. \eqref{eq:quadrature_weights1}-\eqref{eq:quadrature_weights2}, where the weights for the mean and covariance of the state variable are defined as $w^(i)_\mu$ and $w^(i)+\Sigma$ for the $i^{th}$ sigma point.
% \begin{gather}
%     \left[\mathcal{X}\right] = \begin{Bmatrix}\begin{pmatrix}1 \\ 0 \\ . \\ 0\end{pmatrix} & \begin{pmatrix}0 \\ 1 \\  . \\  0\end{pmatrix} & \dots & \begin{pmatrix}0 \\ 0 \\  . \\ 0\end{pmatrix} & \begin{pmatrix}-1 \\ 0 \\ . \\ 0\end{pmatrix}  & \dots \begin{pmatrix}0 \\ 0 \\ . \\ -1\end{pmatrix}\end{Bmatrix} \label{eq:sigma_points} \\
%     \lambda = \alpha^2(d + \kappa) - d \\ 
%     u^{(i)} = \hat{u}^{(i)}\sqrt{d+\lambda},\ \ \forall\hat{u}^{(i)} \in \left[\mathcal{X}\right]
% \end{gather}
% \begin{align}
%    w^{(i)}_\mu &= \begin{cases} \frac{\lambda}{d+\lambda} & \text{i = 0} \\ \frac{1}{2\left(d+\lambda\right)} & \text{i = 1, 2, ..., 2d}\end{cases} \label{eq:quadrature_weights1}\\ 
%    w^{(i)}_\Sigma &= \begin{cases} \frac{\lambda}{d+\lambda}+\left(1 - \alpha^2 + \beta\right) & \text{i = 0} \\ \frac{1}{2\left(d+\lambda\right)} & \text{i = 1, 2, ..., 2d}\end{cases} \label{eq:quadrature_weights2}
% \end{align}
% \subsubsection{Invariant EKF}
% The Invariant Extended Kalman Filter (InEKF) for an underwater vehicle is derived and explained extensively in \cite{potokar_invariant_2021}. The key differences come in the state vector definition, where rather than $\mathbf{x} \in \mathbb{R}^12$ defined in eq. \eqref{eq:state}, it is expressed as $\mathbf{x} \in SE_2(3)$, with according 

% For the EKF and UKF, provide the state transition and measurement models. In another paragraph, write the same models for Invariant EKF.


% \subsubsection{Dense Mapping Methods}
%     The map that is constructed only uses the measurements made from the 1D ping sonar and the DVL. 
%     In order to get a denser output, we use the fact that the DVL is composed of 4 transducers, as shown in fig. \ref{fig:dvl_transducers}.
%     Each of the transducers has an associated altitude measurement.
%     The altitude measurement given by default by the A50 DVL is the single altitude measurement that is an average of these 4 measurements.
%     Instead of using this single measurement made by the DVL, using the output of all 4 sensors will not only lead to a more accurate map but also a denser one.\newline
%     \indent In order to utilize the four transducers, we accounted for the offset and orientation of each of the transducers. These are parameterized as spherical coordinates for the angular offsets, where the radial parameter is simply the range measurement and a translational offset. These offsets are given in table \ref{tab:DVL}.
%     \begin{figure}[H]
%         \centering
%         \captionsetup{justification=centering}
%         \includegraphics[width=0.15 \textwidth]{figures/dvl_transducers.png}
%         \caption{The four transducers of the DVL labeled, along with the coordinate frame of the DVL}
%         \label{fig:dvl_transducers}
%     \end{figure}

%     \begin{table}
%         \captionsetup{justification=centering}
%         \begin{tabular}{|c|c|c|c|}
%         \hline
%         \begin{tabular}[c]{@{}c@{}}Transudcer \\ Number\end{tabular} & Azimuth (${^\circ}$) & Elevation (${^\circ}$) & \begin{tabular}[c]{@{}c@{}}Translation \\ Offset (mm)\end{tabular} \\ \hline
%         1                                                            & 45                   & 22.5                   & (13.86, 13.86, -5.55)                                              \\ \hline
%         2                                                            & 135                  & 22.5                   & (-13.86, 13.86, -5.55)                                             \\ \hline
%         3                                                            & 225                  & 22.5                   & (-13.86, -13.86, -5.55)                                            \\ \hline
%         4                                                            & 315                  & 22.5                   & (13.86, -13.86, -5.55)                                             \\ \hline
%         \end{tabular}
%         \caption{The spherical coordinate parameters to convey the angular offset and translational offset, given as (x, y, z) offers, of the DVL transducers.}
%         \label{tab:DVL}
%     \end{table}



    % \indent Underwater SLAM frameworks, such as \cite{rahman_svin2_2019} and \cite{mallios_ekf-slam_2010} pose the map construction as part of an optimization over the poses of the robot and measured landmarks in the scene.
    % In \cite{mallios_ekf-slam_2010}, a probabilistic scan matching algorithm is used where the pose and measurement uncertainty is used to determine MSIS scans that are loop closure candidates.
    % An essential contribution of our work over \cite{mallios_ekf-slam_2010} is to account for added uncertainty induced by environmental factors in the map.
    % In \cite{rahman_svin2_2019}, the map is constructed as a set of visual features treated as landmarks. 
    % Despite the use of pose and measurement uncertainties in the tightly coupled optimization over the robot poses and landmarks, \cite{rahman_svin2_2019} does not explicitly use either of the uncertainties in the end construction of the map.


    from results:
            % Despite the increased accuracy in the velocity over the robot's operation, we observe that the pose estimate degrades when compared to the baselines without the additive noise. We conducted an in-depth analysis on this finding. From observations of the measurements taken during the wave tests, we observed a persistent bias in the sensor measurements that the DVL was making. This observed bias is shown in Fig. \ref{fig:velocity_bias}, where the ground truth, measured, and estimated velocity are in the $x$-direction in the robot frame. \textbf{TODO: put the filter output from UKF with/without additive noise, get rid of soanr and DVL?}.

        % We argue the downgraded performance of the filters with the additive noises is due to that the filters with the additive noises are less confident with the DVL measurements, which leads to a smaller update step when there is a pulse in its reading. Due to the fact that the number of positive pulses is higher than the number of the negative pulses in DVL readings \textbf{TODO: need to visually or quantitatively report this}, the UKF without the additive noises is benefited from the imbalance and its estimated $v_x$ is closer to the ground truth. 

    
    % The rigidly mounted robot and the linear movement of the carriage give ground truth poses, along with twists to evaluate the performance of the proposed state estimation method. The proposed method for uncertainty-aware state estimation is compared against a standard UKF method that does not include the parameters estimated from the wave experiments as the noise and bias terms.
    %We additionally provide an ablation study to provide insight into each state estimation component's effect. 
     % Figure \ref{fig:3d} shows the estimated 3D trajectory compared to the baseline for the test trial corresponding to measurements in Fig. \ref{fig:plots}.
    
    % We additionally compare the error along the trajectory between the two methods. %Fig. \ref{fig:experiments} provides a qualitative visualization of the error along the trajectory, highlighting major areas of improvement of the proposed methods over the baseline.
    % \subsubsection{Ablation Study}
    %     We perform an ablation study, investigating the individual contribution of the bias estimation and the added noise to the final state estimation. For our ablation study, we build upon the baseline UKF and add components of our proposed method. 
    %     This includes a method that accounts for the bias estimate alone, a method that uses the empirical standard deviation as added noise in the measurement models, a method that uses an empirical standard deviation scaled by a factor of 5 as added noise in the measurement models, and the final proposed method. 
    %     We include the method that has a scaled added noise in order to better highlight the impact of the added noise on the end state estimation results.
    %     The results from the ablation study are shown in Table \ref{tab:ablation}.

        % \subsubsection{Primer on the Counting Sensor Model for OGM}\label{sss:CSM}
    %     The counting sensor model (CSM) is formulated in a Bayesian framework, and the probabilistic representation of the occupancy of the cells is especially useful in the context of uncertainty-aware robotic applications. 
    %     \newline
    %     \indent The objective of CSM is to compute the posterior distribution on the state of the map $\theta$ given sensor measurements $y$: $p(\theta \lvert y)$. 
    %     With each measurement $y$ done sequentially by the robot during its operation, the problem is posed as an incremental Bayesian inference problem.
    %     In this context, $\theta$ is a random variable representing the classification of each cell in the grid $\mathcal{X}$. 
    %     \newline
    %     \indent We define the likelihood function, which is the probability of a sensor measurement $y_i$ given the category of the cell $\theta_j$, as a categorical likelihood, shown in Eqn. \eqref{eq:categorical_likelihood}.
    %     % \begin{gather}
    %     %     p(y_i \lvert \theta_j^k) = \prod_{k=0}^{K-1}\left(\theta_j^{k}\right)^{y_i^k} \label{eq:categorical_likelihood}
    %     % \end{gather}
    %     \indent The prior distribution of $\theta_j$, is taken as a Beta distribution, which is parameterized by the number of categories $K$ and a concentration parameter $\alpha_0 = \{\alpha_0^0, \dots, \alpha_0^K\}$, $\alpha_0^i \in \mathbb{R}_{>0} \forall i$. 
    %     For $K=2$, we notate concentration parameters as $\alpha_0$ and $\beta_0$.
    %     \newline
    %     % \begin{gather}
    %     %     p(\theta_0 | \alpha_0, \beta_0) \sim Beta(K, \alpha_0, \beta_0) = \frac{x^{\alpha_0-1}\left(1-\theta_0\right)^{\beta_0-1}}{B(\alpha_0, \beta_0)} \label{eq:dirichlet} \\
    %     %     B(\alpha, \beta) = \frac{\Gamma(\alpha)\Gamma(\beta)}{\Gamma(\alpha+\beta)}, \quad{} \Gamma(n) = (n-1)! \nonumber
    %     % \end{gather}
    %     \indent Given that the likelihood and prior for this occupancy classification problem are conjugate priors, the posterior distribution belongs to the same family of distribution as the prior, written as a Beta distribution. \newline
    %     \indent This closed form for the posterior allows us to determine what the concentration parameters of the posterior, along with the classification of the cell for category $k$, is. 
    %     The computation of these parameters is given in Eqns. \eqref{eq:parameter_update}-\eqref{eq:posterior_theta}. 
    %     \begin{gather}
    %         \alpha_j := \alpha_0+\sum_{i=1}^Ny_i \quad{} \beta_j := \beta_0+\sum_{i=1}^N(1-y_i) \label{eq:parameter_update} \\
    %         \theta_j^k := \frac{\alpha_j^k-1}{\sum_{k=0}^{K-1}\alpha_j^k - K} \label{eq:posterior_theta}
    %     \end{gather}
    %     We can then compute the mean and variance of $\theta_j$, as shown in Eqn. \eqref{eq:mean_var}.
    %     \begin{gather}
    %         \mathbb{E}[\theta_j]=\frac{\alpha_j}{\alpha_j + \beta_j} \quad{} \mathbb{V}[\theta_j] = \frac{\alpha_j\beta_j}{(\alpha_j+\beta_j)^2(\alpha_j + \beta_j + 1)} \label{eq:mean_var}
    %     \end{gather}
    %     % Hence, using the counting sensor model, we can obtain the exact posterior distribution of the category for each cell, along with it's uncertainty given an altitude measurement from the 1D sonar or DVL. 
